What's in a Smoothness Constant? Tighter Rates for Local SGD with Bounded Second-order Heterogeneity

Local SGD, also known as Federated Averaging, is a widely used distributed optimization algorithm. Although Local SGD often outperforms alternatives such as Mini-batch SGD in practice, theory still only partially explains when and why local updates help under realistic data heterogeneity. Recent work by [Patel et al., 2025] shows that a bounded second-order heterogeneity assumption captures the efficiency of Local SGD for strongly convex objectives, and conjectures that the same principle extends to the general convex setting. In this paper, we prove this conjecture by establishing an improved convergence guarantee for Local SGD on general convex objectives under bounded second-order heterogeneity. We also improve the best-known lower bounds for Local SGD in this setting, showing that our upper bounds are nearly tight. Together, these results provide a sharper, more fine-grained convergence theory for Local SGD. As a further application of our techniques, we provide a lower bound for serial SGD with replacement, showing how second-order heterogeneity captures the impact of rare high-curvature clients.

==> macros.tex <==
\RequirePackage{subcaption}
\usepackage{times}
\usepackage{booktabs}
\usepackage{mdframed}
% \usepackage[textsize=tiny]{todonotes}
\usepackage{bm}
\usepackage{multirow}
\usepackage{tikz}
\usepackage{etoc}
\usetikzlibrary{arrows.meta, positioning, decorations.pathreplacing, calligraphy, shapes, calc, patterns}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepackage{subcaption}
% \usepackage{xcolor=svgnames}
\usepackage{amsmath, amssymb, amsthm, mathtools, natbib}
\usepackage[dvipsnames]{xcolor}
% if you use cleveref..

\usepackage{wrapfig}

\definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{darkred}{rgb}{0.55,0.0,0.0}
\newcommand{\purple}{\color{purple}}
\newcommand{\teal}{\color{teal}}
%\renewcommand{\ttdefault}{cmtt}
\newcommand{\algname}[1]{\texttt{#1}}
%\newcommand{\algname}[1]{{\fontfamily{cmtt}\selectfont #1}}
\newcommand{\algnametitle}[1]{{\sf#1}}
\usepackage[pagebackref]{hyperref}
\usepackage[capitalize,noabbrev]{cleveref}
\hypersetup{
	colorlinks=true,        % false: boxed links; true: colored links
	linkcolor=blue,         % color of internal links
	filecolor=magenta,
	citecolor=darkgreen,         % color of links to bibliography
	urlcolor=blue           % color of external links
}
\renewcommand*{\backrefalt}[4]{%
    \ifcase #1 \footnotesize{(Not cited.)}%
    \or        \footnotesize{(Cited on page~#2)}%
    \else      \footnotesize{(Cited on pages~#2)}%
    \fi}

\usepackage{xspace}
% \usepackage[textsize=scriptsize]{todonotes} % Add the 'disable' flag to 
% \setlength{\marginparsep}{0.2cm} % Changing these seems to have no effect
\setlength{\marginparwidth}{3.5cm}
\usepackage{todonotes}
\newcommand{\ifcomments}{\iftrue}
\newcommand{\kkp}[1]{\todo[color=blue!40,inline]{KKP: #1}\xspace}
\newcommand{\lw}[1]{\todo[fancyline,color=blue!40]{LW: #1}\xspace}
\newcommand{\seb}[1]{\todo[fancyline,color=blue!40]{Seb: #1}\xspace}

\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{oproblem}{Open Problem}
\newtheorem{assumption}{Assumption}
\newtheorem{claim}{Claim}
\newtheorem{lemma}{Lemma}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}

%mathematical operators
\newcommand{\norm}[1]{\left\lVert#1\right\rVert_2}
\newcommand\inner[2]{\left\langle #1, #2 \right\rangle}
\newcommand\ess[0]{\text{ess}}


%vectors
\renewcommand\a[0]{\boldsymbol{a}}
\renewcommand\b[0]{\boldsymbol{b}}
\renewcommand\c[0]{\boldsymbol{c}}
\renewcommand\d[0]{\boldsymbol{d}}
\newcommand\e[0]{\boldsymbol{e}}
\newcommand\f[0]{\boldsymbol{f}}
\newcommand\g[0]{\boldsymbol{g}}
\newcommand\h[0]{\boldsymbol{h}}
\renewcommand\i[0]{\boldsymbol{i}}
\renewcommand\j[0]{\boldsymbol{j}}
\renewcommand\k[0]{\boldsymbol{k}}
\renewcommand\l[0]{\boldsymbol{l}}
\newcommand\m[0]{\boldsymbol{m}}
\newcommand\n[0]{\boldsymbol{n}}
\renewcommand\o[0]{\boldsymbol{o}}
\newcommand\p[0]{\boldsymbol{p}}
\newcommand\q[0]{\boldsymbol{q}}
\renewcommand\r[0]{\boldsymbol{r}}
\newcommand\s[0]{\boldsymbol{s}}
\renewcommand\t[0]{\boldsymbol{t}}
\renewcommand\u[0]{\boldsymbol{u}}
\renewcommand\v[0]{\boldsymbol{v}}
\newcommand\w[0]{\boldsymbol{w}}
\newcommand\x[0]{\boldsymbol{x}}
\newcommand\y[0]{\boldsymbol{y}}
\newcommand\z[0]{\boldsymbol{z}}

%bold letters
\renewcommand\aa[0]{\mathbb{A}}
\newcommand\bb[0]{\mathbb{B}}
\newcommand\cc[0]{\mathbb{C}}
\newcommand\dd[0]{\mathbb{D}}
\newcommand\ee[0]{\mathbb{E}}
\newcommand\ff[0]{\mathbb{F}}
\let\gggg\gg %save the old \gg
% \renewcommand\g[0]{\mathbb{G}}
\newcommand\hh[0]{\mathbb{H}}
\newcommand\ii[0]{\mathbb{I}}
\newcommand\jj[0]{\mathbb{J}}
\newcommand\kk[0]{\mathbb{K}}
\let\llll\ll %save the old \ll
\renewcommand\ll[0]{\mathbb{L}}
\newcommand\mm[0]{\mathbb{M}}
\newcommand\nn[0]{\mathbb{N}}
\newcommand\oo[0]{\mathbb{O}}
\newcommand\pp[0]{\mathbb{P}}
\newcommand\qq[0]{\mathbb{Q}}
\newcommand\rr[0]{\mathbb{R}}
\renewcommand\ss[0]{\mathbb{S}}
%\renewcommand\tt[0]{\mathbb{T}}
\newcommand\uu[0]{\mathbb{U}}
\newcommand\vv[0]{\mathbb{V}}
\newcommand\ww[0]{\mathbb{W}}
\newcommand\xx[0]{\mathbb{X}}
\newcommand\yy[0]{\mathbb{Y}}
\newcommand\zz[0]{\mathbb{Z}}

%cursive letters
\newcommand\aaa[0]{\mathcal{A}}
\newcommand\bbb[0]{\mathcal{B}}
\newcommand\ccc[0]{\mathcal{C}}
\newcommand\ddd[0]{\mathcal{D}}
\newcommand\eee[0]{\mathcal{E}}
\newcommand\fff[0]{\mathcal{F}}
\renewcommand\ggg[0]{\mathcal{G}}
\newcommand\hhh[0]{\mathcal{H}}
\newcommand\iii[0]{\mathcal{I}}
\newcommand\jjj[0]{\mathcal{J}}
\newcommand\kkk[0]{\mathcal{K}}
\renewcommand\lll[0]{\mathcal{L}}
\newcommand\mmm[0]{\mathcal{M}}
\newcommand\nnn[0]{\mathcal{N}}
\newcommand\ooo[0]{\mathcal{O}}
\newcommand\ppp[0]{\mathcal{P}}
\newcommand\qqq[0]{\mathcal{Q}}
\newcommand\rrr[0]{\mathcal{R}}
\newcommand\sss[0]{\mathcal{S}}
\newcommand\ttt[0]{\mathcal{T}}
\newcommand\uuu[0]{\mathcal{U}}
\newcommand\vvv[0]{\mathcal{V}}
\newcommand\www[0]{\mathcal{W}}
\newcommand\xxx[0]{\mathcal{X}}
\newcommand\yyy[0]{\mathcal{Y}}
\newcommand\zzz[0]{\mathcal{Z}}

\newcommand\opt[0]{\x^\star}

%brackets
\newcommand\rb[1]{\left(#1\right)}
\renewcommand\sb[1]{\left[#1\right]}
\newcommand\cb[1]{\left\{#1\right\}}
\newcommand\supp[1]{supp\left(#1\right)}
\newcommand\Exp[0]{\mathbb{E}}

% \usepackage[makeroom]{cancel}

\usepackage{xcolor}
\newcommand{\highlight}[1]{%
	\colorbox{yellow!50}{$\displaystyle#1$}}

\usepackage{lipsum}
\newcommand\NoIndent[1]{%
	\begingroup
	\par
	\parshape0
	#1\par
	\endgroup
}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{booktabs,multirow,colortbl} % for professional tables
\definecolor{headergray}{gray}{0.90}
\definecolor{sectiongray}{gray}{0.96}

\usepackage{adjustbox}

\usepackage{multicol}
\usepackage{colortbl}
\usepackage{xcolor}
